A Convex Approach to Consensus on SO(n)

This paper introduces several new algorithms for consensus over the special orthogonal group. By relying on a convex relaxation of the space of rotation matrices, consensus over rotation elements is reduced to solving a convex problem with a unique global solution. The consensus protocol is then implemented as a distributed optimization using (i) dual decomposition, and (ii) both semi and fully distributed variants of the alternating direction method of multipliers technique -- all with strong convergence guarantees. The convex relaxation is shown to be exact at all iterations of the dual decomposition based method, and exact once consensus is reached in the case of the alternating direction method of multipliers. Further, analytic and/or efficient solutions are provided for each iteration of these distributed computation schemes, allowing consensus to be reached without any online optimization. Examples in satellite attitude alignment with up to 100 agents, an estimation problem from computer vision, and a rotation averaging problem on $SO(6)$ validate the approach.

==> biblio/hscc2.tex <==
@Book{Khalil, author = {Khalil, Hassan}, title = {Nonlinear Systems}, publisher = {Gareth Stevens Pub}, year = {2002}, address = {Milwaukee}, isbn = {9780130673893} }

@INPROCEEDINGS{WP94, 
author={Wicks, M.A. and Peleties, P. and DeCarlo, R.A.}, 
booktitle={Decision and Control, 1994., Proceedings of the 33rd IEEE Conference on}, title={Construction of piecewise Lyapunov functions for stabilizing switched systems}, 
year={1994}, 
month={14-16}, 
volume={4}, 
number={}, 
pages={3492 -3497 vol.4}, 
keywords={ asymptotic stability; piecewise Lyapunov functions; piecewise continuous derivative; sliding mode control; stabilizing switched systems; switched linear systems; system matrices; Lyapunov methods; asymptotic stability; control system analysis; eigenvalues and eigenfunctions; linear systems; matrix algebra; variable structure systems;}, 
doi={10.1109/CDC.1994.411687}, 
ISSN={},}

@article{AL01,
author = {Andrei A. Agrachev and Daniel Liberzon},
collaboration = {},
title = {Lie-Algebraic Stability Criteria for Switched Systems},
publisher = {SIAM},
year = {2001},
journal = siamJCO,
volume = {40},
number = {1},
pages = {253-269},
keywords = {switched system; asymptotic stability; Lie algebra}}

@article{LHM99,
title = {Stability of switched systems: a Lie-algebraic condition},
journal = SCL,
volume = "37",
number = "3",
pages = "117 - 122",
year = "1999",
note = "",
issn = "0167-6911",

author = "Daniel Liberzon and Jo�o P. Hespanha and A. Stephen Morse",
keywords = "Switched system",
keywords = "Uniform exponential stability",
keywords = "Quadratic common Lyapunov function"
}


@INPROCEEDINGS{MMK97,
author={Y. Mori and T. Mori and Y. Kuroe }, 
booktitle= CDC, title={A solution to the common lyapunov function problem for continuous-time systems}, 
year={1997}, 
month={}, 
volume={}, 
number={}, 
pages={3530-3531}, 
}

@INPROCEEDINGS{HespanhaDwellTime,
author={Jo{\~a}o Pedro Hespanha and A.~Stephen Morse }, 
booktitle= CDC, title={Stability of switched systems with average dwell-time}, 
year={1999}, 
month={}, 
volume={3}, 
number={}, 
pages={2655 -2660 vol.3}, 
keywords={average dwell-time;exponential stability;hysteresis-based adaptive control;input-to-state induced norms;nonlinear switched systems;scale-independent hysteresis;slow-on-the-average switching;stable linear systems;supervisory control;switched systems stability;adaptive control;asymptotic stability;hysteresis;linear systems;nonlinear systems;}, 
 
ISSN={},}

@Article{HM02,
  author =       {Jo{\~a}o Pedro Hespanha and A.~Stephen Morse},
  title =        {Switching Between Stabilizing Controllers},
  journal =      Automatica,
  year =         2002,
  volume =       38,
  number =       11,
  pages =        {1905--1917},
  month =        "Nov.",
}

@InProceedings{HM96,
  author =       "Jo{\~a}o Pedro Hespanha and A.~Stephen Morse",
  title =        "Towards the High Performance Control of Uncertain
                  Processes via Supervision",
  volume =       1,
  pages =        "405--410",
  booktitle =    "Proceedings of the Conference on Information Sciences and Systems",
  year =         1996,
  month =        "Mar.",
}

@ARTICLE{FM04, 
title={Information flow and cooperative control of vehicle formations}, 
author={Fax, J.A. and Murray, R.M.}, 
journal=ieeeTAC, 
year={2004}, 
month={Sept.}, 
volume={49}, 
number={9}, 
pages={ 1465-1476}, 
abstract={ We consider the problem of cooperation among a collection of vehicles performing a shared task using intervehicle communication to coordinate their actions. Tools from algebraic graph theory prove useful in modeling the communication network and relating its topology to formation stability. We prove a Nyquist criterion that uses the eigenvalues of the graph Laplacian matrix to determine the effect of the communication topology on formation stability. We also propose a method for decentralized information exchange between vehicles. This approach realizes a dynamical system that supplies each vehicle with a common reference to be used for cooperative motion. We prove a separation principle that decomposes formation stability into two components: Stability of this is achieved information flow for the given graph and stability of an individual vehicle for the given controller. The information flow can thus be rendered highly robust to changes in the graph, enabling tight formation control despite limitations in intervehicle communication capability.}, 
keywords={ control system synthesis, cooperative systems, graph theory, position control, stability, time-varying systems, traffic control, vehicles Nyquist criterion, communication network, communication topology, cooperative control, decentralized information exchange, dynamical systems, formation stability, graph Laplacian matrix, graph theory, information flow, intervehicle communication, multivehicle control}, 
 }

@INPROCEEDINGS{Laf05, 
title={Stable motions of vehicle formations}, 
author={ Williams, A. and Lafferriere, G. and Veerman, J.J.P.}, 
booktitle={Proceedings of the IEEE Conference on Decision and Control and the European Control Conference}, 
year={2005}, 
month={Dec.}, 
volume={}, 
number={}, 
pages={ 72-77}, 
abstract={ We investigate stable maneuvers for a group of autonomous vehicles while moving in formation. The allowed decentralized feeback laws are factored through the Laplacian matrix of the communication graph. We show that such laws allow for stable circular or elliptical motions for certain vehicle dynamics. We find necessary and sufficient conditions on the feedback gains and the dynamic parameters for convergence to formation. In particular, we prove that for undirected graphs there exist feedback gains that stabilize rotational (or elliptical) motions of arbitrary radius (or eceentricity). In the directed graph case we provide necessary and sufficient conditions on the curvature that guarantee stability for a given choice of feedback gains. We also investigate stable motions involving reorientation of the formation along the direction of motion. }, 
keywords={null decentralized control, formation maneuvers , formation stability , graph Laplacian }, 
doi={}, 
ISSN={}, }

@INPROCEEDINGS{Dun07, 
title={Distributed receding horizon control of cost coupled systems}, 
author={Dunbar, W.B.}, 
booktitle=CDC, 
year={2007}, 
month={Dec.}, 
volume={}, 
number={}, 
pages={2510-2515}, 
abstract={This paper considers the problem of distributed control of dynamically decoupled systems that are subject to decoupled constraints, while their states are coupled non- separably in the cost function of an optimal control problem. A distributed receding horizon control (RHC) algorithm is presented, in which each subsystem (agent) computes its own control locally. The implementation presumes synchronous parallel updates. Coupled agents, referred to as neighbors, coordinate by the exchange of an assumed state trajectory prior to each update. The algorithm is an improvement over the previous algorithm developed by the author, in that stability is guaranteed without adding any additional constraints to each local optimal control problem. Instead, a move suppression term is added into each local cost function, which penalizes the deviation of the computed state trajectory from the assumed state trajectory. Closed-loop stability follows if the weight on the move suppression term is larger than a parameter that bounds the amount of coupling in the cost function between neighbors.}, 
keywords={closed loop systems, distributed control, infinite horizon, optimal control, position control, stabilityclosed-loop stability, cost coupled systems, coupled agents, decoupled constraints, distributed control, distributed receding horizon control, dynamically decoupled systems, optimal control problem, state trajectory, synchronous parallel updates}, 
 }

@INPROCEEDINGS{CM03, 
title={Stability analysis of interconnected nonlinear systems under matrix feedback}, 
author={Cremean, L.B. and Murray, R.M.}, 
booktitle=CDC, 
year={2003}, 
month={Dec.}, 
volume={3}, 
number={}, 
pages={ 3078-3083 Vol.3}, 
abstract={ This paper explores the stability analysis problem for nonlinear systems which have general linear feedback interconnections. Systems are often modeled in this manner in the study of decentralized control because many communication topologies can be modeled and analyzed using connections to graph theory. We present necessary conditions for stability of a classification of interconnected systems, and we give some examples to provide insight into this problem. These conditions are related to positive definiteness of matrices associated with the feedback interconnection, and specialize to the common case where the Laplacian matrix of a graph represents the communication topology of the system.}, 
keywords={ decentralised control, feedback, graph theory, interconnected systems, matrix algebra, nonlinear control systems, stability Laplacian matrix, communication topologies, decentralized control, graph theory, interconnected nonlinear systems, linear feedback interconnections, matrix feedback, stability analysis}, 
 }

@ARTICLE{OSM04, 
title={Consensus problems in networks of agents with switching topology and time-delays}, 
author={Olfati-Saber, R. and Murray, R.M.}, 
journal=ieeeTAC, 
year={2004}, 
month={Sept.}, 
volume={49}, 
number={9}, 
pages={ 1520-1533}, 
abstract={ In this paper, we discuss consensus problems for networks of dynamic agents with fixed and switching topologies. We analyze three cases: 1) directed networks with fixed topology; 2) directed networks with switching topology; and 3) undirected networks with communication time-delays and fixed topology. We introduce two consensus protocols for networks with and without time-delays and provide a convergence analysis in all three cases. We establish a direct connection between the algebraic connectivity (or Fiedler eigenvalue) of the network and the performance (or negotiation speed) of a linear consensus protocol. This required the generalization of the notion of algebraic connectivity of undirected graphs to digraphs. It turns out that balanced digraphs play a key role in addressing average-consensus problems. We introduce disagreement functions for convergence analysis of consensus protocols. A disagreement function is a Lyapunov function for the disagreement network dynamics. We proposed a simple disagreement function that is a common Lyapunov function for the disagreement dynamics of a directed network with switching topology. A distinctive feature of this work is to address consensus problems for networks with directed information flow. We provide analytical tools that rely on algebraic graph theory, matrix theory, and control theory. Simulations are provided that demonstrate the effectiveness of our theoretical results.}, 
keywords={ Lyapunov methods, control theory, convergence, delays, graph theory, matrix algebra, time-varying systems Lyapunov functions, control theory, convergence analysis, dynamic agent networks, graph theory, linear consensus protocols, matrix theory, switching topology, time-delays}, }

@ARTICLE{OS06, 
title={Flocking for multi-agent dynamic systems: algorithms and theory}, 
author={Olfati-Saber, R.}, 
journal=ieeeTAC, 
year={2006}, 
month={March}, 
volume={51}, 
number={3}, 
pages={ 401-420}, 
abstract={In this paper, we present a theoretical framework for design and analysis of distributed flocking algorithms. Two cases of flocking in free-space and presence of multiple obstacles are considered. We present three flocking algorithms: two for free-flocking and one for constrained flocking. A comprehensive analysis of the first two algorithms is provided. We demonstrate the first algorithm embodies all three rules of Reynolds. This is a formal approach to extraction of interaction rules that lead to the emergence of collective behavior. We show that the first algorithm generically leads to regular fragmentation, whereas the second and third algorithms both lead to flocking. A systematic method is provided for construction of cost functions (or collective potentials) for flocking. These collective potentials penalize deviation from a class of lattice-shape objects called a-lattices. We use a multi-species framework for construction of collective potentials that consist of flock-members, or a-agents, and virtual agents associated with a-agents called �- and ?-agents. We show that migration of flocks can be performed using a peer-to-peer network of agents, i.e., "flocks need no leaders." A "universal" definition of flocking for particle systems with similarities to Lyapunov stability is given. Several simulation results are provided that demonstrate performing 2-D and 3-D flocking, split/rejoin maneuver, and squeezing maneuver for hundreds of agents using the proposed algorithms.}, 
keywords={ Lyapunov methods, distributed algorithms, multi-agent systems, peer-to-peer computing Lyapunov stability, Reynolds rules, collective potentials, constrained flocking algorithm, cost functions, distributed flocking algorithms, flock members, free-flocking algorithm, lattice-shape objects, multi-agent dynamic systems, multi-species framework, particle systems, peer-to-peer network, split-rejoin maneuver, squeezing maneuver, virtual agents, &alpha,-agents, &alpha,-lattices, &beta,-agents, &gamma,-agents}, 
 }

@ARTICLE{Cort04,
title = {Coverage control for mobile sensing networks},
author = { Cort�s, J. and Mart�nez, S. and Karatas, T. and F. Bullo},
journal = ieeeJRA,  
 year = {2004},
 volume = {20},
 number = {2},
 pages = { 243-255}
 }

@ARTICLE{Bran98, 
title={Multiple Lyapunov functions and other analysis tools for switched and hybrid systems}, 
author={Branicky, M.S.}, 
journal=ieeeTAC, 
year={1998}, 
month={Apr}, 
volume={43}, 
number={4}, 
pages={475-482}, 
abstract={We introduce some analysis tools for switched and hybrid systems. We first present work on stability analysis. We introduce multiple Lyapunov functions as a tool for analyzing Lyapunov stability and use iterated function systems theory as a tool for Lagrange stability. We also discuss the case where the switched systems are indexed by an arbitrary compact set. Finally, we extend Bendixson's theorem to the case of Lipschitz continuous vector fields, allowing limit cycle analysis of a class of �continuous switched� systems}, 
keywords={Lyapunov methods, continuous time systems, control system analysis, limit cycles, nonlinear systems, stability, variable structure systemsBendixson theorem, Lagrange stability, Lipschitz continuous vector, Lyapunov functions, hybrid systems, iterated function systems, limit cycle, nonlinear systems, stability analysis, switched systems, variable structure systems}, 
}



@Article{MP86,
	author = {A. P. Molchanov and E. S. Pyatnitskii},
	title = {Lyapunov functions that define necessary and sufficient conditions for absolute stability of nonlinear nonstationary
control systems. I-II-III},
	year  ={1986},
	journal = {Automat. Remote Control},
	volume = {47},
	pages = {I:344�354, II: 443�451, III:620�630}
}

@INPROCEEDINGS{Shahab, 
author={Kaynama, S. and Oishi, M.}, 
booktitle={Proceedings of the IEEE Conference on Decision and Control and the Chinese Control Conference}, title={Schur-based decomposition for reachability analysis of linear time-invariant systems}, 
year={2009}, 
month={dec.}, 
volume={}, 
number={}, 
pages={69 -74}, 
keywords={Schur based decomposition;complexity reduction;controller synthesis;linear time invariant systems;reachability analysis;reachable sets;control system synthesis;linear systems;reachability analysis;set theory;}, 
}

@book{Lib,
author = {D. Liberzon},
title = {Switching in Systems and Control},
address = { Birkhauser, Boston, MA},
month = { Jun},
year = { 2003},
note = { Volume in series Systems and Control: Foundations and Applications},
} 

@ARTICLE{Rot06, 
title={A characterization of convex problems in decentralized Control*}, 
author={Rotkowitz, M. and Lall, S.}, 
journal=ieeeTAC, 
year={2006}, 
month={Feb.}, 
volume={51}, 
number={2}, 
pages={ 274-286}, 
abstract={ We consider the problem of constructing optimal decentralized controllers. We formulate this problem as one of minimizing the closed-loop norm of a feedback system subject to constraints on the controller structure. We define the notion of quadratic invariance of a constraint set with respect to a system, and show that if the constraint set has this property, then the constrained minimum-norm problem may be solved via convex programming. We also show that quadratic invariance is necessary and sufficient for the constraint set to be preserved under feedback. These results are developed in a very general framework, and are shown to hold in both continuous and discrete time, for both stable and unstable systems, and for any norm. This notion unifies many previous results identifying specific tractable decentralized control problems, and delineates the largest known class of convex problems in decentralized control. As an example, we show that optimal stabilizing controllers may be efficiently computed in the case where distributed controllers can communicate faster than their dynamics propagate. We also show that symmetric synthesis is included in this classification, and provide a test for sparsity constraints to be quadratically invariant, and thus amenable to convex synthesis.}, 
keywords={ closed loop systems, continuous time systems, control system synthesis, convex programming, decentralised control, discrete time systems, feedback, stability closed-loop system, constrained minimum-norm problem, continuous time system, convex problems, convex programming, discrete time system, distributed control, feedback system, optimal decentralized control, quadratic invariance}, 
 }



@phdthesis{FaxThesis,  AUTHOR = {J.A. Fax},  TITLE = {Optimal and cooperative control of vehicle formations},  School= {California Inst. of Techn., Pasadena, CA.},  YEAR = {2002}}

@INPROCEEDINGS{Gupta06, 
title={On the robustness of distributed algorithms}, 
author={Gupta, V. and Langbort, C. and Murray, R.M.}, 
booktitle= CDC, 
year={2006}, 
month={Dec.}, 
volume={}, 
number={}, 
pages={3473-3478}, 
abstract={In recent years, numerous distributed algorithms have been proposed which, when executed by a team of dynamic agents, result in the completion of a joint task. However, for any such algorithm to be practical, one should be able to guarantee that the task is still satisfactorily executed even when agents fail to communicate with others or to perform their designated actions correctly. In this paper, we present a concept of robustness which is well-suited for general distributed algorithms for teams of dynamic agents. Our definition extends a similar notion introduced in the distributed computation literature for consensus problems. We illustrate the definition by considering a variety of algorithms}, 
keywords={distributed algorithmsdistributed algorithms, dynamic agents, robustness}, 
 }



@ARTICLE{Gupta09, 
title={Data Transmission Over Networks for Estimation and Control}, 
author={Gupta, V. and Dana, A.F. and Hespanha, J.P. and Murray, R.M. and Hassibi, B.}, 
journal=ieeeTAC, 
year={2009}, 
month={Aug. }, 
volume={54}, 
number={8}, 
pages={1807-1819}, 
abstract={We consider the problem of controlling a linear time invariant process when the controller is located at a location remote from where the sensor measurements are being generated. The communication from the sensor to the controller is supported by a communication network with arbitrary topology composed of analog erasure channels. Using a separation principle, we prove that the optimal linear-quadratic-Gaussian (LQG) controller consists of an LQ optimal regulator along with an estimator that estimates the state of the process across the communication network. We then determine the optimal information processing strategy that should be followed by each node in the network so that the estimator is able to compute the best possible estimate in the minimum mean squared error sense. The algorithm is optimal for any packet-dropping process and at every time step, even though it is recursive and hence requires a constant amount of memory, processing and transmission at every node in the network per time step. For the case when the packet drop processes are memoryless and independent across links, we analyze the stability properties and the performance of the closed loop system. The algorithm is an attempt to escape the viewpoint of treating a network of communication links as a single end-to-end link with the probability of successful transmission determined by some measure of the reliability of the network.}, 
keywords={closed loop systems, control engineering computing, least mean squares methods, linear quadratic Gaussian control, linear systems, probability, radio links, radio networks, stability, telecommunication network reliability, telecommunication network topology, wireless channelsLQ optimal regulator, arbitrary topology, closed loop system, communication network, data transmission over network, erasure channel, linear time invariant process control, minimum mean squared error method, network reliability, networked control system, optimal linear-quadratic-Gaussian controller, packet-dropping process, probability, remote location, stability, wireless links}, 
 }



@INPROCEEDINGS{Gupta05, 
title={On {LQG} control across a stochastic packet-dropping link}, 
author={ Gupta, V. and Spanos, D. and Hassibi, B. and Murray, R.M.}, 
booktitle= ACC, 
year={2005}, 
month={8-10,}, 
volume={}, 
number={}, 
pages={ 360-365}, 
abstract={}, 
keywords={ Kalman filters, control system synthesis, linear quadratic Gaussian control, optimal control, sensors, stability, state estimation, state feedback, stochastic systems, switched filters Kalman filter, LQG control design, LQR state-feedback, optimal algorithm, optimal linear quadratic Gaussian control, packet drop events, packet drop pattern, sensor-controller communication, separation principle, stochastic packet-dropping link, switched linear filter, unreliable link}, 
}



@INPROCEEDINGS{GHF08, 
title={Coverage control for mobile networks with limited-range anisotropic sensors}, 
author={Gusrialdi, A. and Hatanaka, T. and Fujita, M.}, 
booktitle= CDC, 
year={2008}, 
month={Dec.}, 
volume={}, 
number={}, 
pages={4263-4268}, 
abstract={In this paper the coverage control for mobile sensor networks is studied. The novelty is to consider an anisotropic sensor model where the performance of the sensor depends not only on the distance but also on the orientation from the sensor to the target. Moreover we consider sensors with limited-range sensing defined by a probabilistic model and we assume that each robot is equipped with omni-directional communication capability. A gradient-based distributed algorithm is designed to maximize the joint detection probabilities of the events in the region of interest by the sensors. Simulations illustrate the results.}, 
keywords={mobile radio, probability, robots, telecommunication control, wireless sensor networkscoverage control, gradient-based distributed algorithm, joint detection probabilities, limited-range anisotropic sensors, mobile sensor networks, omni-directional communication capability, robot}, }



@ARTICLE{HS07, 
title={Effective Coverage Control for Mobile Sensor Networks With Guaranteed Collision Avoidance}, 
author={Hussein, I.I. and Stipanovic, D.M.}, 
journal=ieeeTCST, 
year={2007}, 
month={July }, 
volume={15}, 
number={4}, 
pages={642-657}, 
abstract={This paper studies the problem of dynamically covering a given region in the plane using a set of mobile sensor agents. A novel problem formulation is proposed that addresses a number of important multiagent missions. The coverage goal, which is to cover a given search domain using multiple mobile sensors such that each point is surveyed until a certain preset level is achieved, is formulated in a mathematically precise problem statement. A control law is developed that guarantees to meet the coverage goal. This control law is modified to guarantee that a partially connected fleet also attains the coverage goal. Finally, a collision avoidance component is added to the controller to guarantee that the agents do not collide. The new controller is shown to safely achieve coverage. Several numerical examples are provided to illustrate the main results.}, 
keywords={collision avoidance, mobile communication, multi-agent systems, sensors, telecommunication control, wireless sensor networkscollision avoidance, cooperative system, coverage control, mobile sensor agent, mobile sensor network, multiagent missions, multisensor systems},  }




@ARTICLE{Jad03, 
title={Coordination of groups of mobile autonomous agents using nearest neighbor rules}, 
author={Jadbabaie, A. and Jie Lin and Morse, A.S.}, 
journal=ieeeTAC, 
year={2003}, 
month={June}, 
volume={48}, 
number={6}, 
pages={ 988-1001}, 
abstract={ In a recent Physical Review Letters article, Vicsek et al. propose a simple but compelling discrete-time model of n autonomous agents (i.e., points or particles) all moving in the plane with the same speed but with different headings. Each agent's heading is updated using a local rule based on the average of its own heading plus the headings of its "neighbors." In their paper, Vicsek et al. provide simulation results which demonstrate that the nearest neighbor rule they are studying can cause all agents to eventually move in the same direction despite the absence of centralized coordination and despite the fact that each agent's set of nearest neighbors change with time as the system evolves. This paper provides a theoretical explanation for this observed behavior. In addition, convergence results are derived for several other similarly inspired models. The Vicsek model proves to be a graphic example of a switched linear system which is stable, but for which there does not exist a common quadratic Lyapunov function.}, 
keywords={ Lyapunov methods, cooperative systems, distributed control, mobile agents, multi-agent systems Lyapunov function, Viesek model, autonomous agents, discrete-time model, graph theory, mobile autonomous agents, multiagent systems, switched systems}, 
 }

@ARTICLE{Blanchini, 
title={A Separation Principle for Linear Switching Systems and Parametrization of All Stabilizing Controllers}, 
author={Blanchini, F. and Miani, S. and Mesquine, F.}, 
journal=ieeeTAC, 
year={2009}, 
month={Feb. }, 
volume={54}, 
number={2}, 
pages={279-292}, 
abstract={In this paper, we investigate the problem of designing a switching compensator for a plant switching amongst a (finite) family of given configurations (A i,B i,C i). We assume that switching is uncontrolled, namely governed by some arbitrary switching rule, and that the controller has the information of the current configuration i . As a first result, we provide necessary and sufficient conditions for the existence of a switching compensator such that the closed-loop plant is stable under arbitrary switching. These conditions are based on a separation principle, precisely, the switching stabilizing control can be achieved by separately designing an observer and an estimated state (dynamic) compensator. These conditions are associated with (non-quadratic) Lyapunov functions. In the quadratic framework, similar conditions can be given in terms of LMIs which provide a switching controller which has the same order of the plant. As a second result, we furnish a characterization of all the stabilizing switching compensators for such switching plants. We show that, if the necessary and sufficient conditions are satisfied then, given any arbitrary family of compensators Ki(s), each one stabilizing the corresponding LTI plant (A i,B i,C i) for fixed i, there exist suitable realizations for each of these compensators which assure stability under arbitrary switching.}, 
keywords={Lyapunov methods, linear systems, observers, time-varying systemsLMIs, Lyapunov functions, arbitrary switching, closed-loop plant, estimated state compensator, linear switching systems, observer, plant switching, separation principle, sufficient conditions, switching compensator, switching controller, switching rule}, 
 }

@ARTICLE{Rantzer98,
author={Johansson, M. and Rantzer, A.},
journal={Automatic Control, IEEE Transactions on}, title={Computation of piecewise quadratic Lyapunov functions for hybrid systems},
year={1998},
month={Apr.},
volume={43},
number={4},
pages={555 -559},
keywords={Popov criteria;circle criteria;convex optimization;frequency domain;hybrid systems;linear matrix inequality;nonlinear and hybrid systems;piecewise linear systems;piecewise quadratic Lyapunov functions;stability analysis;Lyapunov methods;Popov criterion;matrix algebra;nonlinear systems;optimisation;stability;},
doi={10.1109/9.664157},
ISSN={0018-9286},}


